GumBolt: Extending Gumbel trick to Boltzmann priors

Boltzmann machines (BMs) are appealing candidates for powerful priors in variational autoencoders (VAEs), as they are capable of capturing nontrivial and multi-modal distributions over discrete variables. However, non-differentiability of the discrete units prohibits using the reparameterization trick, essential for low-noise back propagation. The Gumbel trick resolves this problem in a consistent way by relaxing the variables and distributions, but it is incompatible with BM priors. Here, we propose the GumBolt, a model that extends the Gumbel trick to BM priors in VAEs. GumBolt is significantly simpler than the recently proposed methods with BM prior and outperforms them by a considerable margin. It achieves state-of-the-art performance on permutation invariant MNIST and OMNIGLOT datasets in the scope of models with only discrete latent variables. Moreover, the performance can be further improved by allowing multi-sampled (importance-weighted) estimation of log-likelihood in training, which was not possible with previous models.

==> model.tex <==
\\
\begin{figure}[!htbp]
  \centering
  \subfigure[d(q)VAE(++)]{
    \label{fig:dvae}
    \includegraphics[scale=0.35, page=3]{mod_figs.pdf}
  }
  \subfigure[Concrete]{
    \label{fig:concrete}
    \includegraphics[scale=0.35, page=2]{mod_figs.pdf}
  }
  \subfigure[GumBolt]{
    \label{fig:gumbolt}
    \includegraphics[scale=0.35, page=1]{mod_figs.pdf}
  }
  
  \caption[]{
  Schematic of the discussed models with discrete variables in their latent space. The dashed red and solid blue arrows represent the inference network, and the generative model, respectively. (a) dVAE, qVAE \citep{khoshaman2018quantum} and dVAE++ have the same structure. They involve auxiliary continuous variables, $\zeta$, for each discrete variable, $z$, provided by the same conditional probability distribution, $r(\zeta|z)$, in both the generative and approximating posterior networks. (b) Concrete VAE applies the Gumbel trick to the discrete variables to obtain the $\zeta$s that appear in both the inference and generative models. (c) GumBolt only involves discrete variables in the generative model, and the relaxed $\zeta$s are used in the inference model during training. Note that during evaluation, the temperature is set to zero, leading to $\zeta=z$.
    }
  \label{fig:models}
\end{figure}

The importance-weighted or multi-sampled objective of a VAE with BM prior can be written as:
 \begin{equation}
 \begin{split}
      \ML \ge \ELBO{k} &= \Eqi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{p_{\theta}(z^i)p_{\theta}(x|z^i)}{q_\phi(z^i |x)}\right]  \\
      &= \Eqi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{e^{-E_{\theta}(z^i)} p_{\theta} (x|z^i)}{q_\phi(z^i |x)}\right] -\log{Z_{\theta}},
 \end{split}
 \label{eq:ELBO_disc}
 \end{equation} 
where $k$ is the number of samples or importance-weights over which the Monte Carlo objective is calculated,  \citep{mnih2016variational}. Note that we have taken out $Z_\theta$ from the argument of the expectation value, since it is independent of $z$. The partition function is intractable but its derivative can be estimated using sampling:
\begin{equation}
    \nabla_{\theta}\log{Z_{\theta}} = \nabla_{\theta} \log {\sum_{\{z\}}e^{{-E_{\theta}(z)}}} =
     \frac{{\sum_{\{z\}}\nabla_{\theta}  E_{\theta}(z)e^{{-E_{\theta}(z)}}}}{\sum_{\{z\}}e^{{-E_{\theta}(z)}}}
     =
    \underset{p_{\theta} (z)}{\mathbb{E}} 
    \left[ \nabla_{\theta} E_{\theta}(z) \right].   
\label{eq:pf}
\end{equation}

Here, $\sum_{\{z\}}$ involves summing over all possible configurations of the binary vector $z$.
The objective $\ELBO{k}$ cannot be used for training, since it involves indifferentiable discrete variables. This can be resolved by relaxing the distributions:
 \begin{equation}
  \begin{split}
      \ML \ge \Fcont{k} &= \Ezi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{p_\theta(\zeta^i) p_{\theta} (x|\zeta^i)}{q_\phi(\zeta^i |x)}\right] \nonumber \\
      &= \Ezi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{e^{-E_{\theta}(\zeta^i)} p_{\theta} (x|\zeta^i)}{q_\phi(\zeta^i |x)}\right] -\log{\tilde Z_{\theta}}.
 \label{eq:ELBO_cont_full}
  \end{split}
 \end{equation} 
Here, $\zeta^i$ is a continuous variable sampled from  Eq.~\ref{eq:Gumbel}, which is consistent with the Gumbel probability $q_\phi(\zeta^i |x)$ defined in \citep{maddison2016concrete}, and $p_\theta(\zeta) \equiv e^{-E_{\theta}(\zeta)}/\tilde{Z_\theta}$, where $\tilde{Z_\theta} \equiv \int d\zeta e^{-E_{\theta}(\zeta)}$. Notice that $\log \tilde{Z}_\theta$ is different from $\log Z_\theta$, therefore its derivatives cannot be estimated using discrete samples from a BM, making this method inapplicable for BM priors. Analytical calculation of the expectations, suggested for Bernoulli prior in \citep{maddison2016concrete}, is also infeasible for BMs.


\subsection{GumBolt probability proxy}
\label{sec:gumbolt}
To replace $\log \tilde{Z}_\theta$ with $\log Z_\theta$, we introduce a proxy probability distribution:
\begin{equation}
  \breve{p}_{\theta}(\zeta) \equiv \frac{e^{{-E_{\theta}(\zeta)}}}{Z_\theta} .
    \label{eq:gumbolt_p}
\end{equation}


Note that $\breve{p}_{\theta}(\zeta)$ is not a true (normalized) probability distribution, but $\breve{p}_{\theta}(\zeta) \to {p}_{\theta}(z)$ as $\tau \to 0$. 

Now consider the following theorem (see Appendix~\ref{appen:proofgum} for a proof):
 \begin{theorem}
\label{theo:gumbel}
For any polynomial function $E_\theta (z)$ of binary variables $z \in \{0,1\}^{n_z}$, the proxy probability $\breve{p}_{\theta}(\zeta) \equiv e^{-E_\theta (\zeta)}/Z_\theta$, with $\zeta \in [0,1]^{n_z}$, is a lower bound to the true probability ${p}_{\theta}(\zeta)\equiv e^{-E_\theta (\zeta)}/\tilde Z_\theta$, \emph{i.e.}, $\breve{p}_{\theta}(\zeta) \le {p}_{\theta}(\zeta)$, where $Z_{\theta} \equiv {\sum_{\{z\}}{e^{{-E_{\theta}(z)}}}}$ and $\tilde{Z}_\theta \equiv \int\limits_{\{\zeta\}} d\zeta e^{-E_{\theta}(\zeta)}$ .
\end{theorem}

 Therefore, replacing ${p}_{\theta}(\zeta)$ with $\breve{p}_{\theta}(\zeta)$, we obtain a lower bound on $\Fcont{k}$ :
 \begin{equation}
      \F{k} = \Ezi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{e^{-E_{\theta}(\zeta^i)} p_{\theta} (x|\zeta^i)}{q_\phi(\zeta^i |x)}\right] -\log{Z_{\theta}} \le \Fcont{k}.
 \label{eq:ELBO_cont}
 \end{equation} 

This allows reparameterization trick, while making it possible to use sampling to estimate the gradients. The structure of our model with a BM prior is portrayed in Figure~\ref{fig:gumbolt}, where both continuous and discrete variables are used. Notice that in the limit $\tau \to 0$, $\breve{p}_{\theta}(\zeta^i)$ becomes a probability mass function (pmf) $p_\theta(z^i)$, while $q_\phi(\zeta^i |x)$ remains as a probability density function (pdf). To resolve this inconsistency, we replace $q_\phi(\zeta^i |x)$ with the Bernoulli pmf: $\breve{q}_\phi(\zeta^i |x) = \zeta^i \log \bar q^i + (1-\zeta^i) \log (1-\bar q^i)$, which approaches  $q_\phi(z^i |x)$ when $\tau \to 0$. The training objective 
 \begin{equation}
      \Fgumbolt{k} = \Ezi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{e^{-E_{\theta}(\zeta^i)} p_{\theta} (x|\zeta^i)}{\breve{q}_\phi(\zeta^i |x)}\right] -\log Z_\theta
 \label{eq:ELBO_cont}
 \end{equation}
becomes $\ELBO{k}$ at $\tau=0$ as desired (see Fig.~\ref{fig:losses} for the relationship among different objectives). This is the analog of the Gumbel-Softmax trick \citep{jang2016categorical} when applied to BMs.
During training, $\tau$ should be kept small for the continuous variables to stay close to the discrete variables, a common practice with Gumbel relaxation \citep{tucker2017rebar}. For evaluation, $\tau$ is set to zero, leading to an unbiased evaluation of the objective function. 
%In all experiments, detailed in Sec.~\ref{sec:exps}, we use a constant $\tau=\frac{1}{7}$ and observe that the discrete objective follows $\Fgumbolt{k}$ for both training and evaluation, hence no over-fitting and no need for early stopping. 
For generation, discrete samples from BM are directly fed into the decoder to obtain the probabilities of each input feature. 

\subsection{Compatibility of BM with discrete variable relaxation}
\label{sec:stab}
The term in the discrete objective that involves the prior distribution is $\mathbb{E}_{q_\phi(z|x)}\left[ \log p_\theta(z)\right]$. By replacing $z$ with $\zeta$, there is no guarantee that the parameters that optimize $\mathbb{E}_{q_\phi(\zeta|x)}\left[ \log p_\theta(\zeta)\right]$ would also optimize the discrete version. This happens naturally for Bernoulli distribution used in \citep{jang2016categorical}, since the maximum or minimum of $\log (p(\zeta)) = \zeta \log (\bar p) + (1- \zeta) \log(1-\bar p)$ occur at the boundaries (\emph{i.e.}, when $\zeta=1$ or $\zeta=0$). This means that throughout the training, the values of $\zeta$ are pushed towards the boundary points, consistent with the discrete objective. 

In the case of a BM prior, consider the following theorem (proved in Appendix~\ref{appen:proofgum}):
\begin{theorem}
\label{theo:optima_cont_vert}
For any polynomial function $E_\theta (z)$ of binary variables $z \in \{0,1\}^{n_z}$, the extrema of the relaxed function $E_\theta(\zeta)$ with $\zeta \in [0,1]^{n_z}$ reside on the vertices of the hypercube, i.e., $\zeta_{\rm opt} \in \{0,1\}^{n_z}$.
\end{theorem}
Therefore, the maximum or minimum of $\log p_{\theta} (\zeta) \propto -E_{\theta}(z)$, also occur on the boundaries; this shows that having a BM rather than a factorial Bernoulli distribution does not exacerbate the training of GumBolt. 

%It is possible to have a ``straight-through'', \citep{jang2016categorical,gu2015muprop}, version of Eq.~\ref{eq:ELBO_cont} for the $E_{\theta}(\zeta^i)$ term; \emph{i.e.}, when calculating the gradients of this term with respect to $\theta$, the discrete $z^i$ is passed, since the reparametrization trick is not necessary to update the parameters of the generative model. However, we observed empirically that this does not improve the quality of training. See Sec.~\ref{sec:exps} for more details on the experiments.


 
% \begin{algorithm}[h]
% \begin{algorithmic}
% \Require $f(\cdot)$, $\log p(b|\theta)$, reparameterized sampler $b = T(\theta, \epsilon)$, neural network $c_\phi(\cdot)$, \\ \qquad \quad~step sizes $\alpha_1, \alpha_2$ 
% \While {not converged} 
% 	\State $\epsilon \sim p(\epsilon)$ \Comment Sample noise
% 	\State $b \leftarrow T(\epsilon, \theta)$ \Comment Compute input
% 	\State  $\hat g_\theta \leftarrow \left[f(b) - c_{\phi}(b) \right] \nabla_\theta \log p(b|\theta) + \nabla_\theta c_\phi(b)$ \Comment Estimate gradient of objective
% 	\State  $\hat g_\phi \leftarrow \partial \hat g_\theta^2 / \partial \phi$ \Comment Estimate gradient of variance of gradient
% 	\State $\theta \leftarrow \theta - \alpha_1 \hat{g}_\theta$ \Comment Update parameters
% 	\State $\phi \leftarrow \phi - \alpha_2 \hat{g}_\phi$ \Comment Update control variate
% \EndWhile
% \State \textbf{return} $\theta$ 
% \end{algorithmic}
% \caption{GumBolt: Optimizing parameters and a gradient control variate simultaneously.}
% \label{lax}
% \end{algorithm}

 

==> neurips 3/model.tex <==
\\
\begin{figure}[!htbp]
  \centering
  \subfigure[d(q)VAE(++)]{
    \label{fig:dvae}
    \includegraphics[scale=0.35, page=3]{mod_figs.pdf}
  }
  \subfigure[Concrete]{
    \label{fig:concrete}
    \includegraphics[scale=0.35, page=2]{mod_figs.pdf}
  }
  \subfigure[GumBolt]{
    \label{fig:gumbolt}
    \includegraphics[scale=0.35, page=1]{mod_figs.pdf}
  }
  
  \caption[]{
  Schematic of the discussed models with discrete variables in their latent space. The dashed red and solid blue arrows represent the inference network, and the generative model, respectively. (a) dVAE, qVAE \citep{khoshaman2018quantum} and dVAE++ have the same structure. They involve auxiliary continuous variables, $\zeta$, for each discrete variable, $z$, provided by the same conditional probability distribution, $r(\zeta|z)$, in both the generative and approximating posterior networks. (b) Concrete VAE applies the Gumbel trick to the discrete variables to obtain the $\zeta$s that appear in both the inference and generative models. (c) GumBolt only involves discrete variables in the generative model, and the relaxed $\zeta$s are used in the inference model during training. Note that during evaluation, the temperature is set to zero, leading to $\zeta=z$.
    }
  \label{fig:models}
\end{figure}

The importance-weighted or multi-sampled objective of a VAE with BM prior can be written as:
 \begin{equation}
 \begin{split}
      \ML \ge \ELBO{k} &= \Eqi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{p_{\theta}(z^i)p_{\theta}(x|z^i)}{q_\phi(z^i |x)}\right]  \\
      &= \Eqi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{e^{-E_{\theta}(z^i)} p_{\theta} (x|z^i)}{q_\phi(z^i |x)}\right] -\log{Z_{\theta}},
 \end{split}
 \label{eq:ELBO_disc}
 \end{equation} 
where $k$ is the number of samples or importance-weights over which the Monte Carlo objective is calculated,  \citep{mnih2016variational}. Note that we have taken out $Z_\theta$ from the argument of the expectation value, since it is independent of $z$. The partition function is intractable but its derivative can be estimated using sampling:
\begin{equation}
    \nabla_{\theta}\log{Z_{\theta}} = \nabla_{\theta} \log {\sum_{\{z\}}e^{{-E_{\theta}(z)}}} =
     \frac{{\sum_{\{z\}}\nabla_{\theta}  E_{\theta}(z)e^{{-E_{\theta}(z)}}}}{\sum_{\{z\}}e^{{-E_{\theta}(z)}}}
     =
    \underset{p_{\theta} (z)}{\mathbb{E}} 
    \left[ \nabla_{\theta} E_{\theta}(z) \right].   
\label{eq:pf}
\end{equation}

Here, $\sum_{\{z\}}$ involves summing over all possible configurations of the binary vector $z$.
The objective $\ELBO{k}$ cannot be used for training, since it involves indifferentiable discrete variables. This can be resolved by relaxing the distributions:
 \begin{equation}
  \begin{split}
      \ML \ge \Fcont{k} &= \Ezi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{p_\theta(\zeta^i) p_{\theta} (x|\zeta^i)}{q_\phi(\zeta^i |x)}\right] \nonumber \\
      &= \Ezi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{e^{-E_{\theta}(\zeta^i)} p_{\theta} (x|\zeta^i)}{q_\phi(\zeta^i |x)}\right] -\log{\tilde Z_{\theta}}.
 \label{eq:ELBO_cont_full}
  \end{split}
 \end{equation} 
Here, $\zeta^i$ is a continuous variable sampled from  Eq.~\ref{eq:Gumbel}, which is consistent with the Gumbel probability $q_\phi(\zeta^i |x)$ defined in \citep{maddison2016concrete}, and $p_\theta(\zeta) \equiv e^{-E_{\theta}(\zeta)}/\tilde{Z_\theta}$, where $\tilde{Z_\theta} \equiv \int d\zeta e^{-E_{\theta}(\zeta)}$. Notice that $\log \tilde{Z}_\theta$ is different from $\log Z_\theta$, therefore its derivatives cannot be estimated using discrete samples from a BM, making this method inapplicable for BM priors. Analytical calculation of the expectations, suggested for Bernoulli prior in \citep{maddison2016concrete}, is also infeasible for BMs.


\subsection{GumBolt probability proxy}
\label{sec:gumbolt}
To replace $\log \tilde{Z}_\theta$ with $\log Z_\theta$, we introduce a proxy probability distribution:
\begin{equation}
  \breve{p}_{\theta}(\zeta) \equiv \frac{e^{{-E_{\theta}(\zeta)}}}{Z_\theta} .
    \label{eq:gumbolt_p}
\end{equation}


Note that $\breve{p}_{\theta}(\zeta)$ is not a true (normalized) probability distribution, but $\breve{p}_{\theta}(\zeta) \to {p}_{\theta}(z)$ as $\tau \to 0$. 

Now consider the following theorem (see Appendix~\ref{appen:proofgum} for a proof):
 \begin{theorem}
\label{theo:gumbel}
For any polynomial function $E_\theta (z)$ of binary variables $z \in \{0,1\}^{n_z}$, the proxy probability $\breve{p}_{\theta}(\zeta) \equiv e^{-E_\theta (\zeta)}/Z_\theta$, with $\zeta \in [0,1]^{n_z}$, is a lower bound to the true probability ${p}_{\theta}(\zeta)\equiv e^{-E_\theta (\zeta)}/\tilde Z_\theta$, \emph{i.e.}, $\breve{p}_{\theta}(\zeta) \le {p}_{\theta}(\zeta)$, where $Z_{\theta} \equiv {\sum_{\{z\}}{e^{{-E_{\theta}(z)}}}}$ and $\tilde{Z}_\theta \equiv \int\limits_{\{\zeta\}} d\zeta e^{-E_{\theta}(\zeta)}$ .
\end{theorem}

 Therefore, replacing ${p}_{\theta}(\zeta)$ with $\breve{p}_{\theta}(\zeta)$, we obtain a lower bound on $\Fcont{k}$ :
 \begin{equation}
      \F{k} = \Ezi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{e^{-E_{\theta}(\zeta^i)} p_{\theta} (x|\zeta^i)}{q_\phi(\zeta^i |x)}\right] -\log{Z_{\theta}} \le \Fcont{k}.
 \label{eq:ELBO_cont}
 \end{equation} 

This allows reparameterization trick, while making it possible to use sampling to estimate the gradients. The structure of our model with a BM prior is portrayed in Figure~\ref{fig:gumbolt}, where both continuous and discrete variables are used. Notice that in the limit $\tau \to 0$, $\breve{p}_{\theta}(\zeta^i)$ becomes a probability mass function (pmf) $p_\theta(z^i)$, while $q_\phi(\zeta^i |x)$ remains as a probability density function (pdf). To resolve this inconsistency, we replace $q_\phi(\zeta^i |x)$ with the Bernoulli pmf: $\breve{q}_\phi(\zeta^i |x) = \zeta^i \log \bar q^i + (1-\zeta^i) \log (1-\bar q^i)$, which approaches  $q_\phi(z^i |x)$ when $\tau \to 0$. The training objective 
 \begin{equation}
      \Fgumbolt{k} = \Ezi \left[\log \frac{1}{k} \sum_{i=1}^{k} \frac{e^{-E_{\theta}(\zeta^i)} p_{\theta} (x|\zeta^i)}{\breve{q}_\phi(\zeta^i |x)}\right] -\log Z_\theta
 \label{eq:ELBO_cont}
 \end{equation}
becomes $\ELBO{k}$ at $\tau=0$ as desired (see Fig.~\ref{fig:losses} for the relationship among different objectives). This is the analog of the Gumbel-Softmax trick \citep{jang2016categorical} when applied to BMs.
During training, $\tau$ should be kept small for the continuous variables to stay close to the discrete variables, a common practice with Gumbel relaxation \citep{tucker2017rebar}. For evaluation, $\tau$ is set to zero, leading to an unbiased evaluation of the objective function. 
%In all experiments, detailed in Sec.~\ref{sec:exps}, we use a constant $\tau=\frac{1}{7}$ and observe that the discrete objective follows $\Fgumbolt{k}$ for both training and evaluation, hence no over-fitting and no need for early stopping. 
For generation, discrete samples from BM are directly fed into the decoder to obtain the probabilities of each input feature. 

\subsection{Compatibility of BM with discrete variable relaxation}
\label{sec:stab}
The term in the discrete objective that involves the prior distribution is $\mathbb{E}_{q_\phi(z|x)}\left[ \log p_\theta(z)\right]$. By replacing $z$ with $\zeta$, there is no guarantee that the parameters that optimize $\mathbb{E}_{q_\phi(\zeta|x)}\left[ \log p_\theta(\zeta)\right]$ would also optimize the discrete version. This happens naturally for Bernoulli distribution used in \citep{jang2016categorical}, since the maximum or minimum of $\log (p(\zeta)) = \zeta \log (\bar p) + (1- \zeta) \log(1-\bar p)$ occur at the boundaries (\emph{i.e.}, when $\zeta=1$ or $\zeta=0$). This means that throughout the training, the values of $\zeta$ are pushed towards the boundary points, consistent with the discrete objective. 

In the case of a BM prior, consider the following theorem (proved in Appendix~\ref{appen:proofgum}):
\begin{theorem}
\label{theo:optima_cont_vert}
For any polynomial function $E_\theta (z)$ of binary variables $z \in \{0,1\}^{n_z}$, the extrema of the relaxed function $E_\theta(\zeta)$ with $\zeta \in [0,1]^{n_z}$ reside on the vertices of the hypercube, i.e., $\zeta_{\rm opt} \in \{0,1\}^{n_z}$.
\end{theorem}
Therefore, the maximum or minimum of $\log p_{\theta} (\zeta) \propto -E_{\theta}(z)$, also occur on the boundaries; this shows that having a BM rather than a factorial Bernoulli distribution does not exacerbate the training of GumBolt. 

%It is possible to have a ``straight-through'', \citep{jang2016categorical,gu2015muprop}, version of Eq.~\ref{eq:ELBO_cont} for the $E_{\theta}(\zeta^i)$ term; \emph{i.e.}, when calculating the gradients of this term with respect to $\theta$, the discrete $z^i$ is passed, since the reparametrization trick is not necessary to update the parameters of the generative model. However, we observed empirically that this does not improve the quality of training. See Sec.~\ref{sec:exps} for more details on the experiments.


 
% \begin{algorithm}[h]
% \begin{algorithmic}
% \Require $f(\cdot)$, $\log p(b|\theta)$, reparameterized sampler $b = T(\theta, \epsilon)$, neural network $c_\phi(\cdot)$, \\ \qquad \quad~step sizes $\alpha_1, \alpha_2$ 
% \While {not converged} 
% 	\State $\epsilon \sim p(\epsilon)$ \Comment Sample noise
% 	\State $b \leftarrow T(\epsilon, \theta)$ \Comment Compute input
% 	\State  $\hat g_\theta \leftarrow \left[f(b) - c_{\phi}(b) \right] \nabla_\theta \log p(b|\theta) + \nabla_\theta c_\phi(b)$ \Comment Estimate gradient of objective
% 	\State  $\hat g_\phi \leftarrow \partial \hat g_\theta^2 / \partial \phi$ \Comment Estimate gradient of variance of gradient
% 	\State $\theta \leftarrow \theta - \alpha_1 \hat{g}_\theta$ \Comment Update parameters
% 	\State $\phi \leftarrow \phi - \alpha_2 \hat{g}_\phi$ \Comment Update control variate
% \EndWhile
% \State \textbf{return} $\theta$ 
% \end{algorithmic}
% \caption{GumBolt: Optimizing parameters and a gradient control variate simultaneously.}
% \label{lax}
% \end{algorithm}

 
